The gravitational mass of Proxima Centauri measured with SPHERE from a microlensing event

Proxima Centauri, our closest stellar neighbour, is a low-mass M5 dwarf orbiting in a triple system. An Earth-mass planet with an 11 day period has been discovered around this star. The star's mass has been estimated only indirectly using a mass-luminosity relation, meaning that large uncertainties affect our knowledge of its properties. To refine the mass estimate, an independent method has been proposed: gravitational microlensing. By taking advantage of the close passage of Proxima Cen in front of two background stars, it is possible to measure the astrometric shift caused by the microlensing effect due to these close encounters and estimate the gravitational mass of the lens (Proxima Cen). Microlensing events occurred in 2014 and 2016 with impact parameters, the closest approach of Proxima Cen to the background star, of 1\farcs6 $\pm$ 0\farcs1 and 0\farcs5 $\pm$ 0\farcs1, respectively. Accurate measurements of the positions of the background stars during the last two years have been obtained with HST/WFC3, and with VLT/SPHERE from the ground. The SPHERE campaign started on March 2015, and continued for more than two years, covering 9 epochs. The parameters of Proxima Centauri's motion on the sky, along with the pixel scale, true North, and centering of the instrument detector were readjusted for each epoch using the background stars visible in the IRDIS field of view. The experiment has been successful and the astrometric shift caused by the microlensing effect has been measured for the second event in 2016. We used this measurement to derive a mass of 0.150$^{\textrm{+}0.062}_{-0.051}$ (an error of $\sim$ 40\%) \MSun for Proxima Centauri acting as a lens. This is the first and the only currently possible measurement of the gravitational mass of Proxima Centauri.

==> ref_letter.tex <==
While the manuscript presents an interesting result, it suffers from a range of technical shortcomings, which the authors are most strongly encouraged to address.

I particularly note that the exact meaning and interpretation of the quoted uncertainties is never stated (why are some symmetric around the estimated value while others are not?).

The authors should also be more clear about the differences in estimating the mass of Prox Cen with their and other approaches. In particular, they should point out what types of uncertainties play a role. I note that the quoted estimate by Mann et al. (2015) comes with a smaller reported uncertainty than the value claimed by the authors, which might seem to contradict the aim of their investigation.

* The uncertainty on the estimate by Mann et al. (2015) comes from models of mass-luminosity of low-mass stars, which means that the errors are related just on the estimate of the mass itself, and do not include uncertainties from the parallax, or any other property of the star. The estimate that we provide is a completely different measurement, which include all the errors related to the microlensing event, i.e., the distance of the star, proper motions, the instrument calibration errors, etc.  Those two measurements are not comparable in between each other, because they come from two completely different approaches.  

The manuscript is full of acronyms, some of which are never spelt out or explained. Moreover, the captions of tables and figures are generally insufficient for understanding what is shown.

I also note that there a few language issues.

* We spelt out the acronyms, changed the captions and checked the language issues. 

Some further specific comments:

Abstract:
"it is possible to parametrise the microlensing effect" – unclear, what is the point?, should be rephrased

* We rephrased the sentence.

Which objects does the "impact parameter" refer to? Given the bending of light, it should not correspond to the "apparent separation"

* We modified the text.

It would be helpful to the reader to state that gravitational lensing shifts the position, and the size of this shift relates to the mass of the foreground body
"deflection of light .. has been measured" – the deflection and the observed shift in observed position should be distinguished carefully
"for the smallest impact parameter" – unclear

* We modified in the text.

Sect. 1:
Symbol "d" is not defined

* We modified in the text.

"expected shift of the centroid" – please elaborate

* We modified the sentence in the text.

Sect. 2:
"total of 9 epochs were acquired": data were acquired for 9 epochs

* We modified the sentence in the text.

"median combined derotated images cleaned with a spatial filtering" – please provide further detail and/or reference

* We added this sentence:  ``For that we first created a datacube which contains the frames of the observation derotated according to their position angle. Then the median-collapsed image of the cube is produced, after a median filtering that removes isolated high or low values."

Sect. 3:
"fake negative planet technique" – please provide further detail and/or reference

* We added the references where the technique is explained in details.

The last paragraph of Sect. 3.1 preempts the discussion of Sect. 3.2. In fact, the choice of reference frame is most relevant for assessing the motion of Prox Cen. 
With regard to neglecting proper motion and parallax of other stars, how does this effect the final result, and can this be quantified? I note that it one needs to measure "Source 2" relative to Prox Cen. It should be stated explicitly how the trajectory depends on the parameters.

* To estimate the impact of neglecting PM and parallax of the other stars we performed another MCMC with the following data: for each star we created synthetic measurements assuming as RA and Dec at 2016 the median of the RA and Dec from our measurements. The parallax has been given randomly from a uniform distribution between 1 and 3 kpc (we expect these distances for the background stars in the IRDIS FoV), while the PM has been calculated from a gaussian distribution of velocities with sigma of 30 km/s, and random direction. From these synthetic data we derived the parameters of the motion of Proxima, and subsequently, the mass from the microlensing effect. The new value is 0.148 +0.067 -0.055 M_Sun, the fit has a reduced chi square of 0.88. This measurement is consistent with the one that neglects PM and parallax of the background stars.
We included a paragraph in the text.

Sect. 4:
The first subsection of Sect. 4 is missing a title and number.

* We added them.

Eq. (1) describes the "angular Einstein radius", not the "radius of the Einstein ring", which would be D_L θ_E. If the authors are keen on referring to distances, they could note that (4GM)/c^2 equates to twice the Schwarzschild radius of the deflecting body.

* We modified in the text.

Eq. (3) gives an expression for the two images of a point-mass gravitational lens, rather than describing the deflection. The symbol Δθ is not defined. The manuscript is missing a relation between Eq. (3) and the single observed position. 
Where is the routine "AMOEBA" described?

* We added to the text: "AMOEBA is an IDL function which performs a minimum χ-square fit using the downhill simplex method (Nelder & Mead 1965). ''

"reduced chi^2 of 0.87" – What meaning do the authors attach to this? chi^2 should be quoted along with d.o.f.
A description of how the mass of Prox Cen follows from the measurements is missing. What determines the quoted uncertainties?

* The d.o.f. are 14, we added a detailed sentence in the text.

Which star does Sect. 4.3 refer to? The relevance of Sect. 3 is unclear to me.

* We added to the text that we refer to Proxima Cen. 

Sect. 5:
"Einstein radius" -> "angular Einstein radius"

* We changed in the text.

Appendix A:
There is no reference to Appendix A, and it does not contain any text. I do not see any reason why the table should be numbered as A1, rather than in ordinary sequence.

* We moved the Table to the main text. 

Table A1:
The caption does not explain what is shown in this table. What is fitted to what? The meaning of the various quantities is unclear.

* We modified the caption.

Table 1:
Caption is cryptic on the acronyms

* We modified the caption.

Table 2:
It would be helpful to define acronym "TN"

* We modified accordingly.

Table 4:
"offset" relative to what?

* We added a phrase in the caption.

Figure 3:
It should be clarified where the blue line comes from (using a parametric model). It would be instructive to label the epochs

* We added the labels in the Figure and clarified where the blue line comes from.

Figure 4:
Does the shown curve refer to the true positions or the observed positions? How was it constructed?

* We added to the caption: The movement of Proxima on the sky has been calculated using the nominal parameters of parallax and proper motions given by Hipparcos.

Figure 5:
The caption fails to provide a clear description of what is actually shown here? What does the vertical axis of the histograms refer to? What is the meaning of the dashed lines? What do the contours and gray values refer to?
The proper motions are presumably in mas/yr rather than mas (as claimed). It would help to show the units in the figure.
Some numbers are overplotted by lines.

* We rewrote the caption and modified the figure.

Figure 6:
Which "separation" does the plot refer to?
"Results of the measuring the microlensing deflection" – unclear
I fail to understand what is shown in this figure.

* We modified the caption.

